Complex Velocity Structure of Nebular Gas in Active Galaxies Centred in Cooling X-ray Atmospheres

[OII] emission maps obtained with the Keck Cosmic Web Imager (KCWI) are presented for four galaxies centered in cooling X-ray cluster atmospheres. Nebular emission extending tens of kpc is found in systems covering a broad range of atmospheric cooling rates, cluster masses, and dynamical states. Abell 262's central galaxy hosts a kpc-scale disk. The nebular gas in RXJ0820.9+0752 is offset and redshifted with respect to the central galaxy by $10-20$ kpc and 150 km s$^{-1}$, respectively. The nebular gases in PKS 0745-191 and Abell 1835 are being churned to higher velocity dispersion by X-ray bubbles and jets. The churned gas is enveloped by larger scale, lower velocity dispersion (quiescent) nebular emission. The mean line-of-sight speeds of the churned gas, quiescent gas, and the central galaxy each differ by up to $\sim 150$ km s$^{-1}$; nebular speeds upward of $800$ km s$^{-1}$ are found. Gases with outwardly-rising speeds upward of several hundred km s$^{-1}$ are consistent with being advected behind and being lifted by the rising bubbles. The peculiar motion between the galaxy, nebular gas, and perhaps the hot atmosphere from which it presumably condensed is affecting the bubble dynamics, and may strongly affect thermally unstable cooling, the dispersal of jet energy, and the angular momentum of gas accreting onto the galaxies and their nuclear black holes.

==> Comments_referee.tex <==
We greatly appreciate the reviewer's time and valuable comments. They have substantially improved our paper.

The reply to the referee is 


Main comments:
--------------
- I think that this manuscript would considerably gain in quality if (statistical & systematic) uncertainties were assessed - or, at the very least, discussed. This comes with two examples:
1) Figs. 14-17 show a scatter in velocity between spaxels that tends to increase towards the end of the filaments. However, no error bars are displayed and it is difficult to know whether this scatter is really physical or whether it is simply due to uncertainties in the spectra.
   
    We agree and have added error bars to Fig. 14-16, which significantly improves the figures. The addition of the error bars, whose uncertainties come from the uncertainties in v50 from the fits, are mentioned in the second sentence of the 3rd paragraph of Section 4.3.1. 

2) Similarly, high values are seen near the edge of a number of maps (e.g. Fig. 11, as already mentioned in the 2nd paragraph of Sect. 4.2). This makes me suspicious that these "best-fit" measurements are not physical and that their associated errors must be appreciable.

    We have added a new section in the Appendix (Appendix B) that discusses in more depth the uncertainties in the flux and velocity maps. The S/N cuts which we applied to our data ensure that we do not include highly uncertain data; we have also carefully and extensively visually checked the fits to make sure they are robust.

- Somewhat related to my previous comment: in Sect. 2, the authors mention that they assume the metallicity to be solar in their fits. I can easily see why the somewhat uncertain ionization stage of the gas prevents from constraining the metallicity further; however intrinsic metallicity variations may somewhat bias the interpretation of the [O II] emissivity map as tracer of the gas distribution. In turn, I suppose that metallicity under- / over-estimates could also bias the total nebular gas mass estimates displayed in Table 4. Have the authors considered these uncertainties and how they propagate into the quoted estimates?

    As discussed in Section 2.3 step 2, the metallicity is set to solar for the stellar templates which fit the stellar continuum. This is relevant for the fitting of the absorption lines. As seen in Appendix A, we obtain excellent stellar fits with this assumption. As the stellar continuum is well fit, the emission line fits are not substantially affected by the choice of stellar metallicities. We also tested if using stellar templates with different metallicities impacts our results, and they do not; the choice of stellar metallicity in the continuum does not impact the [OII] flux or kinematic maps.

- Although I do appreciate the structure of the Results section (Sect. 3), the authors start by describing Abell 1835 and PKS 0745-191, which are supposedly the two most complex systems of the sample (i.e. multi-components and rather disturbed). In my opinion, restructuring the section and describing the systems by order of simplicity (in particular Abell 262 first, followed by RXJ0820.9+0752, then progressively gain in complexity with the two other systems (Abell 1835 and PKS 0745-191) would make the paper easier to follow and improve its "story-telling".

    We appreciate this point and have reordered the result section as suggested.  We agree that this greatly improves the flow of the paper. Parts of the results section have been edited to respect the continuity of the paper.

- In my opinion, the discussion section (Sect. 4) is interesting but sometimes unnecessarily long. This is especially the case for Sect. 4.4 which sometimes exhibit redundant statements. If possible, I would suggest to restructure this section a bit, to make it somewhat shorter and easier to read.

    We agree that the discussion section was very lengthy and we have significantly shortened it. Fig. 16 in the first version of the paper has been removed, as it did not contribute to the main points of the discussion. The previous section 4.2 was also removed as most of the complex dynamics are seen in Abell 1835 and PKS 0745-191. We also enhanced certain explanations in the discussion section for improved quality. 

- As a non-expert, it is not clear to me how quantities like V_02 and V_95 are derived. I do understand that one (or two) average nebular velocity can be easily derived from the spectrum (which, supposedly, should be dominated by the [OII]3726,9 lines) in each spaxel. However, I would naively assume that deriving V_02 and V_95 would require the knowledge of a full distribution of many velocities in each spaxel, meaning dramatically rich statistics and perfectly known modeling. On the other hand, a simple assumption on the local gas velocity distribution (e.g. following a Gaussian distribution) would result in virtually identical V_02 and V_98 maps (modulo a constant velocity shift). I am aware I must be missing something here, meaning that other readers might be as well. I suggest to clarify this in the main body of the text or in Appendix A (with proper reference in the main body).

    We appreciate this point and have added a more detailed explanation of the calculation of v02 and v98 to the Appendix in Appendix C.1. We also added Fig. 21 which shows emission line fits for the 1 and 2 kinematic component fits. This figure clearly demonstrates how v02 and v98 are defined and shows the relevance of these variables for the two kinematic components fit. The definition of v02 and v98 is also discussed in the first paragraph of Section 3.1.2. 

- Looking at Fig. 3, I am not fully convinced that a second component is necessary. Except perhaps the high velocity spot ~10 kpc E of the nucleus seen in the second component, the two V_50 maps seem to follow each other remarkably well. Moreover, the sigma map of the first component is remarkably flat (and, in fact, at very low velocities), which makes me suspect that this component results from an slight, constant, imperfect line modelling in all spaxels. It seems to me that this could be easily attributed to an instrumental bias rather than some genuine astrophysical component.

    We understand this concern and for Abell 1835 and PKS 0745-191 we added the percentage of the flux which comes from the first and second components, to emphasize that both components are substantial and real (last paragraph of Section 3.3.2). Both components roughly contribute equally to the total emitted flux in regions with two detected kinematic components. We also added a sentence in the 7th paragraph of Section 3.3.2 that refers to Appendix C.2 and Fig. 23 which shows examples of two kinematic component fits. These fits show that the first component does change throughout the galaxy and that it does not come from instrumental bias.

- Looking at Fig. 9, I am surprised by how narrow the high-sigma "filament" is compared to the radio jet. I think it would be important to determine whether this is an instrumental effect (e.g. if the radio beam is ~10' large). If not, this would have important implications as it would mean that turbulence injected by the central AGN is more efficiently collimated than the diffusion of accelerated electrons.

    We have updated Fig. 3 to add the beam size of the 1.4 GHz VLA observation in the lower right of the figure. We also added a few sentences in the last paragraph of Section 3.1.2 to mention how the highest sigma gas coincides with the brightest 1.4 GHz radio emission.


Minor comments:
---------------


- The point the authors make in the 8th paragraph of Sect. 3.2.2 (on the interpretation of sigma as caused by difference of velocities) is excellent. It demonstrates that sigma should *not* necessarily interpreted as small-scale motions, in praticular turbulence. This point is valid well outside optical wavelength (e.g. interpretation of high-resolution X-ray spectra with XRISM). I suggest to emphasize it a little more in the paper.

    The 7th and 8th paragraphs of Section 3.4.2 highlight the importance of disentangling the 1st and 2nd kinematic components. This text discusses how when different kinematic components of the nebular gas are present total sigma maps can be misleading as large sigma values can be caused by large differences in the v50 of the different kinematic components.

- Unlike what is claimed in the 3rd paragraph of Sect. 4.6, Table 4 does not contain the values of M_mol. I think it would be useful to add them in that table.

    We fixed the reference for Mmol values in the second paragraph of Section 4.5.

- Do I understand correctly that, in Abell 1835 and PKS 0745-191, the "first" component corresponds to the dominant one in terms of flux? If so, to avoid confusion, I would suggest to rename "first" and "second" components into, respectively "primary" and "secondary" components.

    The terms "first" and "second" components does not indicate that one is brightest or more important than the other. The relative flux of the first and second component varies throughout the [OII] emission maps. This can be seen in Figures 23 and 25 in Appendix C. This is mentioned at different places throughout the text.

- In Eq. (3), isn't a "[OII]" superscript missing near the f_i term of the denominator?

    This has been fixed.

- In the last paragraph of Sect. 4.5, M_mol is mentioned but not explicitly defined (although it is easy to guess that it corresponds to the mass of molecular gas). For completeness, I suggest to define this quantity explicitly.

    The definition of Mmol is now defined in the notes of Table 1.

- In Fig. 7, I suggest to add a pair of arrows to indicate the direction of the cavities.

    We considered this and concluded that adding arrows to Fig. 1 would make the figure crowded. Instead we added a comment about the position of the cavities and refer the reader to Fig. 3 in the figure caption.

- In the 2nd paragraph of Sect. 3.3, "4 kpc" should not be written in math mode.

    This has been fixed.

- In the last paragraph of Sect. 3.4 (before Sect. 3.4.1), 10^{10} M. should be 10^{10} $M_\odot$.

    This has been fixed.

Other remarks:

We have also added/edited a few additional items in the text. Such changes include editing Fig. 12 which was partially showing incorrect data and the associated text in the discussion. We also added in Appendix A the non-corrected systemic redshifts for our targets, which can be useful for future comparison with our results.
